Structure-based Anomaly Detection and Clustering

Anomaly detection is a fundamental problem in domains such as healthcare, manufacturing, and cybersecurity. This thesis proposes new unsupervised methods for anomaly detection in both structured and streaming data settings. In the first part, we focus on structure-based anomaly detection, where normal data follows low-dimensional manifolds while anomalies deviate from them. We introduce Preference Isolation Forest (PIF), which embeds data into a high-dimensional preference space via manifold fitting, and isolates outliers using two variants: Voronoi-iForest, based on geometric distances, and RuzHash-iForest, leveraging Locality Sensitive Hashing for scalability. We also propose Sliding-PIF, which captures local manifold information for streaming scenarios. Our methods outperform existing techniques on synthetic and real datasets. We extend this to structure-based clustering with MultiLink, a novel method for recovering multiple geometric model families in noisy data. MultiLink merges clusters via a model-aware linkage strategy, enabling robust multi-class structure recovery. It offers key advantages over existing approaches, such as speed, reduced sensitivity to thresholds, and improved robustness to poor initial sampling. The second part of the thesis addresses online anomaly detection in evolving data streams. We propose Online Isolation Forest (Online-iForest), which uses adaptive, multi-resolution histograms and dynamically updates tree structures to track changes over time. It avoids retraining while achieving accuracy comparable to offline models, with superior efficiency for real-time applications. Finally, we tackle anomaly detection in cybersecurity via open-set recognition for malware classification. We enhance a Gradient Boosting classifier with MaxLogit to detect unseen malware families, a method now integrated into Cleafy's production system.

==> chapters/copyright_releases.tex <==
\chapter{Copyright releases}
    \label{cha:copyright_releases}
    
    \lettrine{C}{opyright releases}.
    

==> chapters/quotes/ending_quote.tex <==
\setlength\epigraphwidth{6.275cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Not all those who wander are lost''\footnotemark}}}{}
\footnotetext{Gandalf, \emph{The Lord of the Rings: The Fellowship of the Ring} by J.R.R. Tolkien}


==> chapters/quotes/quotes.tex <==
\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``But in the end, it's only a passing thing, this shadow. Even darkness must pass. A new day will come. And when the sun shines it will shine out the clearer.''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Two Towers}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Don't adventures ever have an end? I suppose not. Someone else always has to carry on the story.''}}}{{\small{--- \textup{Bilbo Baggins}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``I expect they had lots of chances, like us, of turning back, only they didn't. And if they had, we shouldn't know, because they'd have been forgotten.''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Two Towers}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``This is it. If I take one more step, it'll be the farthest away from home I've ever been.''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``There's some good in this world, Mr. Frodo, and it's worth fighting for.''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Two Towers}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``All we have to decide is what to do with the time that is given us.''}}}{{\small{--- \textup{Gandalf}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``I wish it need not have happened in my time,'' said Frodo. ``So do I,'' said Gandalf, ``and so do all who live to see such times. But that is not for them to decide. All we have to decide is what to do with the time that is given us.''}}}{{\small{--- \textup{Frodo Baggins and Gandalf}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Our people, our people. I would have followed you, my brother... my captain... my king.''}}}{{\small{--- \textup{Gandalf}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``I made a promise, Mr Frodo. A promise. `Don't you leave him Samwise Gamgee.' And I don't mean to. I don't mean to.''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Many that live deserve death. And some that die deserve life. Can you give it to them? Then do not be too eager to deal out death in judgement. For even the very wise cannot see all ends.''}}}{{\small{--- \textup{Gandalf}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``I know what I must do. It's just... I'm afraid to do it.''}}}{{\small{--- \textup{Frodo Baggins}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``In this phial,'' she said, ``is caught the light of Eärendil's star, set amid the waters of my fountain. It will shine still brighter when night is about you. May it be a light to you in dark places, when all other lights go out.''}}}{{\small{--- \textup{Galadriel}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``I will not say: do not weep; for not all tears are an evil.''}}}{{\small{--- \textup{Gandalf}, \emph{The Lord of the Rings: The Return of the King}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Do you remember the Shire, Mr. Frodo? It'll be spring soon. And the orchards will be in blossom. And the birds will be nesting in the hazel thicket. And they'll be sowing the summer barley in the lower fields... and eating the first of the strawberries with cream. Do you remember the taste of strawberries?''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Return of the King}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``It's like the great stories, Mr. Frodo, the ones that really mattered. Full of darkness and danger they were, and sometimes you didn't want to know the end because how could the end be happy? How could the world go back to the way it was when so much bad has happened? But in the end, it's only a passing thing this shadow, even darkness must pass. A new day will come, and when the sun shines, it'll shine out the clearer. I know now folks in those stories had lots of chances of turning back, only they didn't. They kept going because they were holding on to something. That there's some good in this world, Mr. Frodo, and it's worth fighting for.''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Two Towers}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``But in the end, it's only a passing thing, this shadow. Even darkness must pass. A new day will come. And when the sun shines it will shine out the clearer.''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Two Towers}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Come, Mr. Frodo!'' he cried. ``I can't carry it for you, but I can carry you.''}}}{{\small{--- \textup{Samvise Gamgee}, \emph{The Lord of the Rings: The Return of the King}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``A wizard is never late, nor is he early, he arrives precisely when he means to.''}}}{{\small{--- \textup{Gandalf}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``The world isn't in your books and maps, it's out there.''}}}{{\small{--- \textup{Gandalf}, \emph{The Hobbit}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``True courage is about knowing not when to take a life, but when to spare one.''}}}{{\small{--- \textup{Gandalf}, \emph{The Hobbit}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Saruman believes it is only great power that can hold evil in check, but that is not what I have found. It is the small everyday deeds of ordinary folk that keep the darkness at bay. Small acts of kindness and love.''}}}{{\small{--- \textup{Gandalf}, \emph{The Hobbit}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``I didn't think it would and this way.'' said Pippin. ``End? No, the journey doesn't end here. Death is just another path, one that we all must take. The grey rain-curtain of this world rolls back, and all turns to silver glass, and then you see it.'' said Gandalf. ``What? Gandalf? See what?''. ``White shores, and beyond, a far green country under a swift sunrise.''. ``Well, that isn't so bad.''. ``No. No, it isn't.''.}}}{{\small{--- \textup{Pippin and Gandalf Gamgee}, \emph{The Lord of the Rings: The Return of the King}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``It is not despair, for despair is only for those who see the end beyond all doubt. We do not. It is wisdom to recognize necessity, when all other courses have been weighed, though as folly it may appear to those who cling to false hope. Well, let folly be our cloak, a veil before the eyes of the Enemy! For he is very wise, and weighs all things to a nicety in the scales of his malice. But the only measure that he knows is desire, desire for power; and so he judges all hearts. Into his heart the thought will not enter that any will refuse it, that having the Ring we may seek to destroy it. If we seek this, we shall put him out of reckoning.''}}}{{\small{--- \textup{Gandalf}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``May the wind under your wings bear you where the sun sails and the moon walks.''}}}{{\small{--- \textup{Gandalf}, \emph{The Hobbit}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``It is not our part to master all the tides of the world, but to do what is in us for the succour of those years wherein we are set, uprooting the evil in the fields that we know, so that those who live after may have clean earth to till. What weather they shall have is not ours to rule.''}}}{{\small{--- \textup{Gandalf}, \emph{The Lord of the Rings: The Return of the King}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``There are many things in the deep waters; and seas and lands may change. And it is not our part here to take thought only for a season, or for a few lives of Men, or for a passing age of the world. We should seek a final end of this menace, even if we do not hope to make one.''}}}{{\small{--- \textup{Gandalf}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Memory is not what the heart desires. That is only a mirror.''}}}{{\small{--- \textup{Gimli}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Don't adventures ever have an end? I suppose not. Someone else always has to carry on the story.''}}}{{\small{--- \textup{Bilbo Baggins}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Such is of the course of deeds that move the wheels of the world: small hands do them because they must, while the eyes of the great are elsewhere.''}}}{{\small{--- \textup{Elrond}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}

\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``It is no bad thing to celebrate a simple life.''}}}{{\small{--- \textup{Bilbo Baggins}, \emph{The Lord of the Rings: The Fellowship of the Ring}}}}


\setlength\epigraphwidth{6.125cm}
\setlength\epigraphrule{0pt}
\epigraph{{\large \emph{``Frodo wouldn't have got far without Sam.'' said Frodo. ``Now Mr. Frodo, you shouldn't make fun; I was being serious.'' said Sam. ``So was I.''}}}{{\small{--- \textup{Frodo Baggins and Samvise Gamgee}, \emph{The Lord of the Rings: The Two Towers}}}}
